SSF: Sparse Long-Range Scene Flow for Autonomous Driving

Scene flow enables an understanding of the motion characteristics of the environment in the 3D world. It gains particular significance in the long-range, where object-based perception methods might fail due to sparse observations far away. Although significant advancements have been made in scene flow pipelines to handle large-scale point clouds, a gap remains in scalability with respect to long-range. We attribute this limitation to the common design choice of using dense feature grids, which scale quadratically with range. In this paper, we propose Sparse Scene Flow (SSF), a general pipeline for long-range scene flow, adopting a sparse convolution based backbone for feature extraction. This approach introduces a new challenge: a mismatch in size and ordering of sparse feature maps between time-sequential point scans. To address this, we propose a sparse feature fusion scheme, that augments the feature maps with virtual voxels at missing locations. Additionally, we propose a range-wise metric that implicitly gives greater importance to faraway points. Our method, SSF, achieves state-of-the-art results on the Argoverse2 dataset, demonstrating strong performance in long-range scene flow estimation. Our code will be released at https://github.com/KTH-RPL/SSF.git.

==> sections/limitations.tex <==
% Three notable limitations of our proposed method merit discussion. 
\section{Limitations} \label{sec:limitations}

==> tables/effect_voxel_size.tex <==
\begin{table*}[h]
\centering
% \scriptsize
\def\arraystretch{1.2}
\setlength{\tabcolsep}{3.0pt}
\caption{Analyzing the effect of voxel size on scene flow performance. The grid size is set to $102.4 \times 102.4$~\si{m}. FPS denotes the frame rate for inference. As the voxel size is reduced, the memory goes up and frame rate reduces drastically for FastFlow3D and DeFlow. On the other hand, our method, SSF, maintains a constant memory and frame rate.}
\label{tab:voxel_size}
\begin{tabular}{cc|ccccc|cc|c|c}
\toprule
  \multirow{2}{*}{Methods} & \multirow{2}{*}{Voxel size (\si{m})} & \multicolumn{5}{c|}{Three-way EPE} & \multicolumn{2}{c|}{Bucket-Normalized EPE} & \multirow{2}{*}{Memory (MB) ↓} & \multirow{2}{*}{FPS ↑} \\
                           &            & Mean ↓       & EPE FD ↓ & EPE FS ↓ & EPE BS ↓ & Dy. IOU ↑ & Dy. Mean ↓ & Static Mean ↓ & &  \\ 
\hline
\multirow{3}{*}{FastFlow3D} & 0.2   & 0.0508 & \textbf{0.0077} & 0.0198 & 0.1248 & 0.6202 & 0.4314  & 0.0160 & 1736 & 38.26  \\

& 0.1   & 0.0411 & \underline{0.0078} & \textbf{0.0169} & 0.0986 & 0.6904 & 0.3389 & 0.0152 & 4616 & 12.73   
\\

& 0.075 & 0.0435 & 0.0102 & 0.0179 & 0.1025 & 0.6659 & 0.3371 & 0.0172 & 7556 & 7.68   
\\
\hline 

\multirow{3}{*}{DeFlow}     & 0.2   & 0.0392 & 0.0080 & 0.0221 & 0.0876  & 0.6325 & 0.3279 & 0.0186 & 1732 & 30.52  
\\

& 0.1   & 0.0368 & 0.0078 & 0.0211 & 0.0815 & 0.6587 & 0.2782 & 0.0185 & 4620 & 11.71   \\

& 0.075 & 0.0374 & 0.0078 & 0.0219 & 0.0823 & 0.6523 & 0.2814 & 0.0195 & 7556 & 7.21   
\\
\hline

\multirow{3}{*}{SSF (Ours)}        & 0.2   & 0.0364 & 0.0083 & 0.0173 & 0.0837 & 0.6627 & 0.2330 & 0.0149 & 2610 & 43.58  
\\

& 0.1   & \textbf{0.0343} & \textbf{0.0077} & 0.0172 & \underline{0.0778} & \textbf{0.7007} & \textbf{0.1962} & \textbf{0.0137} & 2610 & 43.25  
\\

& 0.075 & \underline{0.0345} & 0.0088 & \underline{0.0171} & \textbf{0.0775} & \underline{0.6997} & \underline{0.2013} & \underline{0.0140} & 2610 & 43.66
 \\
\bottomrule
  % Add more rows here
\end{tabular}
\end{table*}


==> tikz/1D532054-768E-486D-BA06-30FB3C390865.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={time},
xmajorgrids,
xmin=0, xmax=10,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Speed (m/s)},
ymajorgrids,
ymin=0, ymax=40,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0 6.71202471234191
0.1 6.71212650413523
0.2 6.71320161601858
0.3 6.71571971145201
0.4 6.72183766613334
0.5 6.73019302157916
0.6 6.73637694780359
0.7 6.72831439055839
0.8 6.71658761051972
0.9 6.70353010039088
1 6.6863083361169
1.1 6.66520356688714
1.2 6.6440739385626
1.3 6.62353394143528
1.4 6.6017390364367
1.5 6.57822516287673
1.6 6.55181858610996
1.7 6.5219881844951
1.8 6.48901217213124
1.9 6.45498217609582
2 6.42040472652682
2.1 6.38526597797995
2.2 6.34992393769454
2.3 6.31412754569929
2.4 6.27744069368862
2.5 6.24047579420392
2.6 6.20405040538093
2.7 6.16831099291595
2.8 6.13411080999295
2.9 6.1026085199839
3 6.07311337720809
3.1 6.04354817574024
3.2 6.01410066576357
3.3 5.98582675756972
3.4 5.96039648180083
3.5 5.93806514067297
3.6 5.91911989930222
3.7 5.90475938790188
3.8 5.89680292266841
3.9 5.89657942828985
4 5.90445939137127
4.1 5.92026693720539
4.2 5.94128418761199
4.3 5.96563960412441
4.4 5.99103220459708
4.5 6.01673836495861
4.6 6.04336436986499
4.7 6.07123543054912
4.8 6.10108892359348
4.9 6.13269345316793
5 6.16502124783009
5.1 6.19818676420169
5.2 6.23143479438893
5.3 6.26512614059627
5.4 6.29889951798765
5.5 6.33149212548943
5.6 6.36319048658953
5.7 6.3941031046647
5.8 6.42466041855346
5.9 6.45407135865259
6 6.48203266028448
6.1 6.50831679308746
6.2 6.53295258396727
6.3 6.55656184321725
6.4 6.57919820833863
6.5 6.6028206709945
6.6 6.62858816637784
6.7 6.65684960347955
6.8 6.68759273171915
6.9 6.72078231273906
7 6.75635494153552
7.1 6.79435742714861
7.2 6.83354901874738
7.3 6.87346262441178
7.4 6.91390608843172
7.5 6.95462994766928
7.6 6.99505008793036
7.7 7.03345227754504
7.8 7.06504824964518
7.9 7.08821522010447
8 7.10257934442056
8.1 7.10862388162113
8.2 7.10856420733003
8.3 7.10853153423777
};
\addlegendentry{MHE}
\addplot [semithick, darkorange25512714]
table {%
0 6.50924695475223
0.1 6.77862505903709
0.2 6.57466667111938
0.3 6.73709675686949
0.4 6.00555144567131
0.5 6.18860032793027
0.6 6.19155846094841
0.7 10.4031983765258
0.8 6.28092210486421
0.9 6.29285667271901
1 7.40369869457888
1.1 7.42492895200204
1.2 6.3447902097414
1.3 6.35252199190382
1.4 6.9063558320403
1.5 6.72180178408042
1.6 6.94588659326776
1.7 6.97126227138414
1.8 7.00301521405625
1.9 6.43704061691167
2 6.46731306302387
2.1 6.50809036336751
2.2 6.33841326911777
2.3 6.37447281182024
2.4 6.49167319867468
2.5 6.31905883012231
2.6 6.13093823637765
2.7 6.20854166157762
2.8 6.04958433796676
2.9 5.6823597438689
3 5.74522187628929
3.1 6.2978029289496
3.2 6.11672020503744
3.3 5.95702334340392
3.4 5.57851957383552
3.5 5.66322777366265
3.6 5.69505841771691
3.7 5.52870104860443
3.8 5.20742053071722
3.9 5.03235669975401
4 5.03533632683853
4.1 4.86202752806491
4.2 5.49694352765755
4.3 5.56715262362991
4.4 6.03194432026411
4.5 6.09996080477162
4.6 5.90382291269483
4.7 5.96854085522395
4.8 5.77286240968193
4.9 5.84912304273175
5 6.17001890434511
5.1 5.99934653557052
5.2 6.30827714112921
5.3 6.12178191947726
5.4 6.17354025451713
5.5 6.56666000579845
5.6 6.40003574507065
5.7 6.46327933457758
5.8 6.30537084236629
5.9 6.58478096363733
6 6.60807294110667
6.1 6.675068428527
6.2 6.72940990446505
6.3 6.57634495339401
6.4 6.83851640014947
6.5 6.3985883750721
6.6 6.30040362364653
6.7 6.33987820909524
6.8 6.39914758423188
6.9 6.43878886541034
7 6.49241253530109
7.1 6.38845069281766
7.2 6.75455174956129
7.3 6.78998577595216
7.4 6.81123091701026
7.5 6.84662511636138
7.6 6.86786527920537
7.7 6.88916615650134
7.8 8.03334067848102
7.9 8.03619033996073
8 8.05843708869443
8.1 8.10888080106935
8.2 8.1132128096501
8.3 8.15288156239514
};
\addlegendentry{Naive}
\end{axis}

\end{tikzpicture}

